Cosmological constraints from harmonic space analysis of DES Y3 3x2 clustering

The large-scale distribution of matter, as mapped by photometric surveys like the Dark Energy Survey (DES), serves as a powerful probe into cosmology. It is especially sensitive to both the amplitude of matter clustering ($\sigma_8$) and the total matter density ($\Omega_m$). The fiducial analysis of the two-point clustering statistics of these surveys is invariably done in configuration space where complex masking scheme is easier to handle. However, such an analysis inherently mixes different scales together, requiring special care in modeling. In this study, we present an analysis of DES Y3 3x2 clustering data in harmonic space where small and large scales are better separated and can be neatly modeled using perturbative techniques. Using conservative scale cuts together with Limber approximation and a Gaussian covariance assumption in a first study, we model the clustering data under a linear bias model for galaxies, incorporating comprehensive treatment for astrophysical effects. We subsequently extend this fiducial analysis to explore a third-order biasing prescription. For our fiducial analysis, we get $S_8=0.789\pm0.020$, consistent with the configuration space analysis presented by the DES collaboration, although under our different modeling choices, we find a preference for a lower $\Omega_m$ and a higher $\sigma_8$. The analysis sets the stage for a future search for signatures of primordial non-Gaussianity and blue-tilted isocurvature perturbations from photometric surveys.

==> old_theory.tex <==
\section{Theory}
In this section, we provide expressions for the galaxy-galaxy ($C_{ij}^{gg}(l)$), cosmic shear ($C_{ij}^{\gamma\gamma}(l)$) and galaxy-galaxy lensing ($C_{ij}^{g\gamma}(l)$) spectra. \commentout{in terms of the 3D matter powerspectrum $P_{mm}$.} 

The angular power spectrum of projected galaxy number density in terms of 3D galaxy power spectrum $P_{gg}$ is an oscillatory integral in three variables and is given by
\begin{align}
C_{ij}^{gg}(l) &= \int \frac{d\chi}{\chi} \, \frac{d\chi'}{\chi'} \, \frac{2k^2 \, dk}{\pi} \, W^g_i(\chi) W^g_i(\chi') \nonumber \\ 
&\times  j_l(k\chi) j_l(k\chi') P_{gg}(k,\chi,\chi')  \label{eq:clff_exact}
\end{align}
where $W_i^g$ is a weight function given by
\begin{equation}
    W_i^{g}(\chi) = H(\chi(z)) n(\chi(z))
\end{equation}
and $P_{gg}$ is galaxy powerspectrum which is a complex function of primordial field but under linear galaxy bias model, which is valid on the largest scales, it can be expressed as
\begin{equation}
    P_{gg}^{ij}(k, \chi, \chi') = b^ib^j P_{mm}(k, \chi, \chi')
\end{equation}
The observed galaxy angular powerspectrum $C_{ij}^{gg}(l)$ has additional contribution from redshift-space distortions (RSD) and lens magnification, details of which could be found in \cite{DES:2021rex}. In our analysis, we ignore RSD effects which has negligible impact for DES Y3 \cite{DES:2021rex} and include a constant bias model with for modelling magnification of lens galaxies.


The lensing potential $\psi$ at a given position ($\vec{\theta}$) in the sky is a projection of 3D Newtonian potential $\Phi$
\begin{equation}
    \psi(\vec{\theta}) = 2 \int \frac{d\chi}{\chi} \Phi(\chi, \vec{\theta}\chi) q(\chi)
\end{equation}
where $q$ is called the lensing efficiency
\begin{equation}
    q(\chi) = \int d\chi' n(\chi') \frac{\chi' - \chi}{\chi}
\end{equation}
The lensing efficiency $q$ encodes information about the geometry of the Universe. The 3D potential is related to the matter field via the Poisson equation. The second orderr derivatives of the lensing potential defines the shear $\Gamma$ and convergence $\kappa$
The shear field $\gamma = \gamma_1 + i\gamma_2$ is a spin 2 field and is related to the potential via
\begin{equation*}
    \kappa = \frac{1}{4}(\eth \bar{\eth} + \bar{\eth} \eth )\psi(\vec{\theta}); \ \ \  \ \ \ \gamma(\vec{\theta}) = \frac{1}{2} \eth \eth \psi(\vec{\theta}) \nonumber \\
\end{equation*}
\begin{align}
    \kappa &= (\psi_{11} + \psi_{22})/2 \nonumber \\
    (\gamma_1, \gamma_2) &= \big((\psi_{11} - \psi_{22})/2, (\psi_{12} + \psi_{21})/2 \big)
\end{align}
%where the convergence $\kappa$ is given by 
%\begin{equation}
%    \kappa = \frac{3\Omega_mH_0^2}{2}\int_0^\chi \frac{d\chi'}{\chi'} \bigg( \frac{\chi - \chi'}{\chi\chi'} \bigg) \delta(\chi'\theta, \chi')
%\end{equation}
In this paper, we work in the harmonic space where the shear $\gamma$ can be equivalently expressed in terms of spin-weighted spherical harmonics basis $_sY_{lm}$
\begin{equation}
    \gamma(\theta) = -\sum_{lm} _{\pm2}Y_{lm}(E_{lm} \pm iB_{lm})
\end{equation}
where $E$ and $B$ are the curl-free and divergence-free modes. 
The gravitational induced $E$-mode power spectrum is related to convergence as
\begin{equation}
    C_{EE}(l) = G(l)^2 C_{\kappa\kappa}(l)
\end{equation}
where $G_l$ is an $l$-dependent spin-prefactor given by
\begin{equation}
    G(l) = \frac{\ellbar}{(l+1/2)^2} = \frac{1}{(l+1/2)^2}\sqrt{\frac{(l+2)!}{(l-2)!}}
\end{equation}
for the spin-2 shear field. The prefactor is $\sim 1$ for $l\sim\mathcal{O}(10)$.
%\commentout{
%The shear $\gamma$ can be equivalently expressed in terms of spin-weighted spherical harmonics basis $_sY_{lm}$
%\begin{equation}
%    \gamma(\theta) = -\sum_{lm} _{\pm2}Y_{lm}(E_{lm} \pm iB_{lm})
%\end{equation}
%where E and B are the curl-free and divergence-free modes. 
%Using the above relation, one can write the full spherical shear powerspectrum in terms of lensing potential and 3D matter powerspectrum as follows.
%\begin{align}
%    C_{ij}^{\gamma\gamma}(l) &= \frac{1}{4}\ellbar^2(l,2)C_{ij}^{\psi\psi} \nonumber \\
%    &= \frac{2}{\pi}\ellbar^2(l,2) [\frac{3}{2}\Omega_m\frac{H_0}{c}]^2 \times \nonumber \\
%    & \int \frac{d\chi}{\chi} \int\frac{d\chi'}{\chi'} \int \frac{dk}{k^2} P_{mm}(k, \chi\theta) j_l(k\chi)j_l'(k\chi')
%\end{align}
%}
\vspace{0.25cm}

For Stage-III photometric surveys, the fast and efficient Limber approximation of the above integral is sufficiently accurate for $l>40$. \commentout{The 3x2 two-point statistics includes galaxy-galaxy, galaxy-galaxy lensing and lensing power spectra.} Under this approximation, the auto and cross powerspectrum $C_{AB}^{ij}(l)$ for two tracers $A$ and $B$ for tomographic bins $i$ and $j$ can be written as \cite{limber, loverde2008extended}
\begin{equation*}
    C^{AB}_{ij}(l) = \int \frac{d\chi}{\chi^2} W_A^i(\chi) W_B^j(\chi) P_{AB}\bigg(k=\frac{l+1/2}{\chi},\ z(\chi)\bigg)
\end{equation*}
where $W_A^i$ is a kernel enconding the weight specific to a tracer $A$ for tomographic bin $i$. \commentout{For galaxy number counts, this is given by the galaxy number density i.e.\ $W_g^{i}(\chi)=n^i_g(z(\chi)$.} 

For the $E$-mode, the kernel has a slightly complex form given by
\begin{equation}
    W_\gamma^i(\chi) \equiv G_l \frac{3}{2}H_0^2\Omega_m \frac{\chi}{a(\chi)}\int dz' n_s^i(z') \bigg[\frac{\chi(z')-\chi}{\chi(z')}\bigg]
\end{equation}
where $n_s^i$ is the source galaxy number density for bin $i$. \sai{Note that the factor $G_l\rightarrow1$ for $\ell>O(10)$.} Although our discussion is in terms of auto spectrum, it is straightforwardly generalized to get expressions for cross spectra as well.  %and $G_l$ is an $l$-dependent spin-prefactor given by
%\begin{equation}
%    G(l) = \frac{\ellbar}{(l+1/2)^2} = \frac{1}{(l+1/2)^2}\sqrt{\frac{(l+2)!}{(l-2)!}}
%\end{equation}
%for the spin-2 shear field. The prefactor is $\sim 1$ for $l\sim\mathcal{O}(10)$.

